D-Aug: Enhancing Data Augmentation for Dynamic LiDAR Scenes

Creating large LiDAR datasets with pixel-level labeling poses significant challenges. While numerous data augmentation methods have been developed to reduce the reliance on manual labeling, these methods predominantly focus on static scenes and they overlook the importance of data augmentation for dynamic scenes, which is critical for autonomous driving. To address this issue, we propose D-Aug, a LiDAR data augmentation method tailored for augmenting dynamic scenes. D-Aug extracts objects and inserts them into dynamic scenes, considering the continuity of these objects across consecutive frames. For seamless insertion into dynamic scenes, we propose a reference-guided method that involves dynamic collision detection and rotation alignment. Additionally, we present a pixel-level road identification strategy to efficiently determine suitable insertion positions. We validated our method using the nuScenes dataset with various 3D detection and tracking methods. Comparative experiments demonstrate the superiority of D-Aug.

==> draft.tex <==
\begin{table}
\caption{Units for Magnetic Properties}
\label{table}
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{|p{25pt}|p{75pt}|p{110pt}|}
\hline
Symbol& 
Quantity& 
Conversion from Gaussian and \par CGS EMU to SI$^{\mathrm{a}}$ \\
\hline
$\Phi $& 
Magnetic flux& 
1 Mx $\to  10^{-8}$ Wb $= 10^{-8}$ V $\cdot$ s \\
$B$& 
Magnetic flux density, \par magnetic induction& 
1 G $\to  10^{-4}$ T $= 10^{-4}$ Wb/m$^{2}$ \\
$H$& 
Magnetic field strength& 
1 Oe $\to  10^{-3}/(4\pi )$ A/m \\
$m$& 
Magnetic moment& 
1 erg/G $=$ 1 emu \par $\to 10^{-3}$ A $\cdot$ m$^{2} = 10^{-3}$ J/T \\
$M$& 
Magnetization& 
1 erg/(G $\cdot$ cm$^{3}) =$ 1 emu/cm$^{3}$ \par $\to 10^{-3}$ A/m \\
4$\pi M$& 
Magnetization& 
1 G $\to  10^{-3}/(4\pi )$ A/m \\
$\sigma $& 
Specific magnetization& 
1 erg/(G $\cdot$ g) $=$ 1 emu/g $\to $ 1 A $\cdot$ m$^{2}$/kg \\
$j$& 
Magnetic dipole \par moment& 
1 erg/G $=$ 1 emu \par $\to 4\pi \times  10^{-10}$ Wb $\cdot$ m \\
$J$& 
Magnetic polarization& 
1 erg/(G $\cdot$ cm$^{3}) =$ 1 emu/cm$^{3}$ \par $\to 4\pi \times  10^{-4}$ T \\
$\chi , \kappa $& 
Susceptibility& 
1 $\to  4\pi $ \\
$\chi_{\rho }$& 
Mass susceptibility& 
1 cm$^{3}$/g $\to  4\pi \times  10^{-3}$ m$^{3}$/kg \\
$\mu $& 
Permeability& 
1 $\to  4\pi \times  10^{-7}$ H/m \par $= 4\pi \times  10^{-7}$ Wb/(A $\cdot$ m) \\
$\mu_{r}$& 
Relative permeability& 
$\mu \to \mu_{r}$ \\
$w, W$& 
Energy density& 
1 erg/cm$^{3} \to  10^{-1}$ J/m$^{3}$ \\
$N, D$& 
Demagnetizing factor& 
1 $\to  1/(4\pi )$ \\
\hline
\multicolumn{3}{p{251pt}}{Vertical lines are optional in tables. Statements that serve as captions for 
the entire table do not need footnote letters. }\\
\multicolumn{3}{p{251pt}}{$^{\mathrm{a}}$Gaussian units are the same as cg emu for magnetostatics; Mx 
$=$ maxwell, G $=$ gauss, Oe $=$ oersted; Wb $=$ weber, V $=$ volt, s $=$ 
second, T $=$ tesla, m $=$ meter, A $=$ ampere, J $=$ joule, kg $=$ 
kilogram, H $=$ henry.}
\end{tabular}
\label{tab1}
\end{table}


\begin{figure}
\centerline{\includegraphics[width=\columnwidth]{fig1.png}}
\caption{Magnetization as a function of applied field. Note that ``Fig.'' is abbreviated. There is a period after the figure number, followed by two spaces. It is good practice to explain the significance of the figure in the caption.}
\end{figure}



==> related_work.tex <==
\section{Related Works}
\textbf{Data Augmentation}
Data augmentation, a crucial technique in deep learning, plays an essential role in enhancing the generalization ability of neural networks by artificially expanding the diversity and quantity of training samples. This strategy is particularly significant in the context of 3D point cloud data, often used in applications like autonomous driving and 3D object detection. Global data augmentations, like rotation, flip, and scaling~\cite{Yan_Mao_Li_2018, Lang_Vora_Caesar_Zhou_Yang_Beijbom_2019, Shi_Guo_Jiang_Wang_Shi_Wang_Li_2020, Shi_Wang_Li_2019, He_Zeng_Huang_Hua_Zhang_2020}, are common across 3D point-cloud neural networks. These techniques, by altering the geometrical perspective, contribute to a more diverse set of training samples. Additionally, automation of augmentation strategies~\cite{cheng2020improving}, as proposed in various studies, can narrow the search space for optimal augmentations based on previous training iterations. Another data augmentation strategy is called object augmentation. One of the early methods in this realm was GT-Aug, introduced within the 3D detection model SECOND~\cite{Yan_Mao_Li_2018, Yin_Zhou_Krahenbuhl_2021}. GT-Aug operates by adding samples from a precomputed ground-truth database to the training scene. However, it overlooks aspects such as collision handling, visibility, and occlusion of inserted scan points. In contrast, LiDAR-Aug~\cite{Fang_Zuo_Zhou_Jin_Wang_Zhang_2021}, another state-of-the-art technique, offers a more sophisticated approach. It not only enriches training data by rendering additional objects based on CAD models but also accounts for occlusion between these objects and the scene. Unlike GT-Aug, LiDAR-Aug includes simulations of interactions between objects, providing a more realistic augmentation. In comparison to the state-of-the-art LiDAR-Aug,  the bounding box generation of Real3D-Aug~\cite{vsebek2022real3d} allows for the augmentation of semantic segmentation datasets and simulates real occlusions in the entire spherical projection. The inserted augmentations come from the same dataset and are placed at the same distance, ensuring natural reflectance values and point distribution, including ray dropouts.

\textbf{Data Simulation}
Further addressing the challenge of data collection and labeling, which is both resource-intensive and time-consuming, synthetic data simulations like SYNTHIA~\cite{Ros_Sellart_Materzynska_Vazquez_Lopez_2016} offer diverse urban scene images with comprehensive annotations. Video games, notably Grand Theft Auto V, are also employed for generating ground truth data in training models~\cite{Richter_Hayder_Koltun_2017, Richter_Vineet_Roth_Koltun_2016, Yue_Wu_Seshia_Keutzer_Sangiovanni-Vincentelli_2018}. This trend extends to using advanced driving simulators for creating a variety of labeled data. Despite these advancements, bridging the domain gap between synthetic and real data remains an ongoing focus. Techniques such as image translation through GANs~\cite{Sallab_Sobh_Zahran_Essam_2019, Sallab_Sobh_Zahran_Shawky_2019} and merging real-world imagery with virtual objects~\cite{Debevec_2008,li2019aads} have been explored to enhance the realism and applicability of synthesized data. In LiDAR simulation, innovative approaches like inserting synthetic CADs into real backgrounds~\cite{Fang_Zhou_Yan_Zhao_Zhang_Ma_Wang_Yang_2020} and using the reconstructed dynamic objects from point cloud instead of synthetic CADs~\cite{Manivasagam_Wang_Wong_Zeng_Sazanovich_Tan_Yang_Ma_Urtasun_2020} further exemplify the evolving strategies to make synthetic data more realistic and useful for complex applications like autonomous driving.

\textbf{3D Object Detection} In the domain of LiDAR point cloud processing, which is pivotal for applications like autonomous driving and advanced 3D object detection, researchers face challenges such as the inherent sparsity of data, unstructured nature of point clouds, and varying point densities. In exploring 3D object detection more broadly, it is evident that there are two main streams: those relying solely on point clouds~\cite{Yan_Mao_Li_2018, Chen_Liu_Zhang_Qi_Jia, Yin_Zhou_Krahenbuhl_2021} where methods can be categorized into projection/view-based~\cite{Ku_Mozifian_Lee_Harakeh_Waslander_2018, Yang_Luo_Urtasun_2018, Luo_Yang_Urtasun_2018, Zhou_Fang_Song_Guan_Yin_Dai_Yang_2019, Hu_Ziglar_Held_Ramanan_2020}, voxel-based~\cite{Kuang_Wang_An_Zhang_Zhang_2020, Yin_Shen_Guan_Zhou_Yang_2020, Zhou_Tuzel_2018, Chen_Liu_Zhang_Qi_Jia, Yan_Mao_Li_2018}, and raw point cloud-based~\cite{Zhou_Fang_Song_Guan_Yin_Dai_Yang_2019, Lang_Vora_Caesar_Zhou_Yang_Beijbom_2019, Qi_Liu_Wu_Su_Guibas_2018} approaches. And those integrating multiple sensor modalities~\cite{vora2020pointpainting,yoo20203d,chen2017multi}. By applying our data augmentation technique to various representative detection methods such as CenterPoint~\cite{Yin_Zhou_Krahenbuhl_2021}, VoxelNeXt~\cite{Chen_Liu_Zhang_Qi_Jia}, TransFusion-L~\cite{transfusion}, and PointPillars~\cite{pointpillars}, among other methods, we aim to demonstrate the efficacy and adaptability of our augmentation method. This comprehensive evaluation underscores the versatility of our approach in enhancing feature representation and object detection performance across a suite of leading models.%上面的例子可能得改一下

\textbf{3D Object Tracking}
3D object tracking models, essential for applications like autonomous driving, create tracks for multiple objects across multi-frame LiDAR data. Traditional methods~\cite{Benbarka_Schroder_Zell_2021, Chiu_Li_Ambrus_Bohg_2021, Weng_Wang_Held_Kitani_2020} primarily use the Kalman filter for processing detection results, as seen in AB3DMOT~\cite{Weng_Wang_Held_Kitani_2020}. More recent models, such as CenterPoint~\cite{Yin_Zhou_Krahenbuhl_2021}, enhance tracking by predicting object velocities to associate centers across consecutive frames, a concept based on the foundational principles of CenterTrack~\cite{Zhou_Koltun_Krähenbühl_2020}.
In the context of VoxelNeXt~\cite{Chen_Liu_Zhang_Qi_Jia}, the integration of query voxels for association marks a significant enhancement in tracking accuracy by addressing the prediction bias typically associated with the estimation of object centers. Considering that state-of-the-art LiDAR point cloud data augmentation techniques like LiDAR-Aug~\cite{Fang_Zuo_Zhou_Jin_Wang_Zhang_2021} and Real3D-Aug~\cite{vsebek2022real3d} predominantly focus on single-frame augmentation, they fall short for 3D object tracking that necessitates an understanding of temporal relationships across multiple frames. Our paper introduces a dynamic augmentation approach that is inherently more versatile and aptly suited for the complexities of multi-frame 3D object tracking.
